Model Hubs and Beyond: Analyzing Model Popularity, Performance, and Documentation

With the massive surge in ML models on platforms like Hugging Face, users often lose track and struggle to choose the best model for their downstream tasks, frequently relying on model popularity indicated by download counts, likes, or recency. We investigate whether this popularity aligns with actual model performance and how the comprehensiveness of model documentation correlates with both popularity and performance. In our study, we evaluated a comprehensive set of 500 Sentiment Analysis models on Hugging Face. This evaluation involved massive annotation efforts, with human annotators completing nearly 80,000 annotations, alongside extensive model training and evaluation. Our findings reveal that model popularity does not necessarily correlate with performance. Additionally, we identify critical inconsistencies in model card reporting: approximately 80% of the models analyzed lack detailed information about the model, training, and evaluation processes. Furthermore, about 88% of model authors overstate their models' performance in the model cards. Based on our findings, we provide a checklist of guidelines for users to choose good models for downstream tasks.

==> figures/perf_tweet_eval_evaluate_easy.tex <==
\begin{figure*}[!htb]
     \centering
     \includegraphics[width=\textwidth]{assets/barplot_te_be_vbw_app.pdf}
     \caption{Performance scores (F1) of first 100 models in $M_{500}$, organized in descending order. These scores correspond to easy instances of the $\mathcal{D}_{t}$ under the Evaluate strategy. Model names corresponding to Model IDs can be found in Table~\ref{tab:m100_models} in the \S\ref{sec:appendix}.}
     \label{fig:te_eval_easy}
\end{figure*}

% barplot_te_be_vbw_app
% barplot_te_be_vbw
